Algorithms as Social-Ecological-Technological Systems: an Environmental Justice Lens on Algorithmic Audits

This paper reframes algorithmic systems as intimately connected to and part of social and ecological systems, and proposes a first-of-its-kind methodology for environmental justice-oriented algorithmic audits. How do we consider environmental and climate justice dimensions of the way algorithmic systems are designed, developed, and deployed? These impacts are inherently emergent and can only be understood and addressed at the level of relations between an algorithmic system and the social (including institutional) and ecological components of the broader ecosystem it operates in. As a result, we claim that in absence of an integral ontology for algorithmic systems, we cannot do justice to the emergent nature of broader environmental impacts of algorithmic systems and their underlying computational infrastructure. We propose to define algorithmic systems as ontologically indistinct from Social-Ecological-Technological Systems (SETS), framing emergent implications as couplings between social, ecological, and technical components of the broader fabric in which algorithms are integrated and operate. We draw upon prior work on SETS analysis as well as emerging themes in the literature and practices of Environmental Justice (EJ) to conceptualize and assess algorithmic impact. We then offer three policy recommendations to help establish a SETS-based EJ approach to algorithmic audits: (1) broaden the inputs and open-up the outputs of an audit, (2) enable meaningful access to redress, and (3) guarantee a place-based and relational approach to the process of evaluating impact. We operationalize these as a qualitative framework of questions for a spectrum of stakeholders. Doing so, this article aims to inspire stronger and more frequent interactions across policymakers, researchers, practitioners, civil society, and grassroots communities.

==> tables/table_questions.tex <==
\begin{table}[]
\caption{Socio-ecological-technical strategies vs. emerging thematic considerations within the field of environmental justice}
\label{tab:overview-table}
\begin{tabular}{ p{2cm}p{4cm}p{4cm}p{4cm}  }
 %\begin{tabular}[h!]{ |p{2cm}||p{3cm}|p{3cm}|p{3cm}|  }
 \hline
 \setlength{\tabcolsep}{25pt}
  & Practice and materiality & Community, identity, and attachment & Human and non-human assemblages\\ [0.5ex] 
 \hline\hline
 
 \setlength{\tabcolsep}{25pt}
Broadening the inputs and outputs of the assessment 
 & \emph{Who decides what data, knowledges, and other factors are taken into account as inputs in conducting an impact assessment? How are the outputs of an impact assessment integrated in other processes (i.e. policy, business models, capacity building)? }
 & \emph{How do we ensure legitimacy of the non-Western knowledge systems that could contribute to an impact assessment?
What happens with the outcomes of an impact assessment? How are they shared and what decisions are made based on them in the local context where they are deployed?
}
 & \emph{Who represents natural ecosystems? How is the consideration of non-human natural entities taken into account in the set of inputs of an algorithmic impact assessment? } 
 \\ 
 \hline
De-centering to cede power in frontline communities
& \emph{Are there civil society and grassroot communities which we could meaningfully engage with in designing and implementing algorithmic impact assessment process?  How do we ensure that frontline communities have access to the inputs and outputs of an impact assessment?}
& \emph{How are local communities where an algorithmic system is deployed participating in the algorithmic impact assessment process? How are they rewarded for their participation? How is their individual and collective identity and agency acknowledged and taken into account?}
& \emph{Could we consult with environmental ethicists, environmental scientists, environmental lawyers, civil society organizations, or other stakeholders who could provide a critical lens for the pragmatic approach to the impact assessment?}
\\
 \hline
Adopting a place-based and relational approach 
& \emph{How are the characteristics of a particular place taken into account in the algorithmic impact assessment process with regards to the local resources, ecosystem services, and services to ecosystems.}
& \emph{What is the relationship between the algorithmic impact assessment process and local communities and their territories, local environmental ecosystems, and cultural heritage taken into account?}
& \emph{How is the relationship between human and non-human actors incorporated in the impact assessment process? How is it impacted by its outputs?} \\ [1ex]
 %\hline
 %5 & 88 & 788 & 6344 \\ [1ex] 
 \hline
\end{tabular}
\label{table:1_overview}
\end{table}
